An Embarrassingly Simple Approach for Transfer Learning from Pretrained Language Models

A growing number of state-of-the-art transfer learning methods employ language models pretrained on large generic corpora. In this paper we present a conceptually simple and effective transfer learning approach that addresses the problem of catastrophic forgetting. Specifically, we combine the task-specific optimization function with an auxiliary language model objective, which is adjusted during the training process. This preserves language regularities captured by language models, while enabling sufficient adaptation for solving the target task. Our method does not require pretraining or finetuning separate components of the network and we train our models end-to-end in a single step. We present results on a variety of challenging affective and text classification tasks, surpassing well established transfer learning methods with greater level of complexity.

==> naaclhlt2019/tex/akn.tex <==
\section{Acknowledgements}
We would like to thank Katerina Margatina and Georgios Paraskevopoulos for their helpful suggestions and comments. This work has been partially supported by  computational time granted from the Greek Research \& Technology Network  (GR-NET) in the National HPC facility - ARIS. Also, the authors
would like to thank NVIDIA for supporting this
work by donating a TitanX GPU. 

==> naaclhlt2019/tex/conclusions.tex <==
\section{Conclusions and Future Work}

We introduce SiATL, a simple and efficient transfer learning method for text classification tasks.  Our approach is based on pretraining a LM and  transferring its weights to a classifier with a task-specific layer. The model is trained using a task-specific functional with an auxiliary LM loss. 
SiATL avoids catastrophic forgetting of the language distribution learned by the pretrained LM. Experiments on various text classification tasks
%Twitter and general corpora
yield results competitive to the state-of-the-art, demonstrating the efficacy of our approach. Furthermore, our method outperforms more sophisticated transfer learning approaches, such as ULMFiT in all tasks.

In  future work, we plan to incorporate subword information in our LMs and experiment with bidirectional architectures. Furthermore, we plan to pretrain LMs on generic corpora. Finally, we will investigate adaptive schemes for sequential unfreezing and $\gamma$ decay over training epochs.

% \hl{++future}
% In the future we plan to experiment with ...

==> naaclhlt2019/tex/exp.tex <==
\section{Results \& Discussion}


\noindent\textbf{Baselines and Comparison.}  Table \ref{table:results} summarizes our results. The top two rows detail the baseline performance of the BoW and NBoW models. We observe that when enough data is available (e.g. \textit{Sent17}), baselines provide decent results. Next, the results for the generic classifier initialized from a pretrained LM (P-LM) are shown with and without sequential unfreezing, followed by the results of the proposed model SiATL. SiATL is also directly compared with its close relative ULMFiT (trained on Wiki-103 or Twitter) and the state-of-the-art for each task; ULMFiT also  fine-tunes a LM for classification tasks. The proposed SiATL method consistently outperforms the baselines, the P-LM method and  ULMFiT in all datasets. Even though we do not perform any elaborate learning rate scheduling and we limit ourselves to pretraining in Twitter, we obtain higher results in two Twitter datasets and three generic. 

 \begin{figure}[!t]
 \centering
 \resizebox{.8\columnwidth}{!}{%
	\captionsetup{farskip=0pt} % no gap at the top
	\centerline{\includegraphics[width=1.1\columnwidth]{images/plot_gamw_to_kerato_mou_mesa_gamw}}\\
	} 
	\resizebox{0.85\columnwidth}{!}{%
	\captionsetup{farskip=0pt} % no gap at the top
	\centerline{\includegraphics[width=1.2\columnwidth]{a}}\\

	}
	\caption{Results of our proposed approach (SiATL) (o) and ULMFiT (+) for different datasets as a function of the number of training examples. }
\label{few}
\end{figure}







\noindent\textbf{Auxiliary LM objective.}
The effect of the auxiliary objective is highlighted in very small datasets, such as \textit{SCv1}, where it results in an impressive boost in performance (7\%). We hypothesize that when the classifier is simply initialized with the pretrained LM, it overfits quickly, as the target vocabulary is very limited. The auxiliary LM loss, however, permits refined adjustments to the model and fine-grained adaptation to the target task. 

\noindent\textbf{Exponential decay of $\gamma$.}
For the optimal $\gamma$ interval, we empirically find that exponentially decaying $\gamma$ to half
of its initial value over the number of training epochs provides best results for our classification tasks. A heatmap of $\gamma$ is depicted in Figure \ref{fig:heatmap}. We observe that small values of $\gamma$ should be employed, in order to scale the LM loss in the same order of magnitude as the classification loss over the training period. 

\noindent\textbf{Sequential Unfreezing.}
Results show that sequential unfreezing is crucial to the proposed method, as it allows the pretrained LM to adapt to the target word distribution. 
%, which is likely to be very different from the source LM distribution. 
The performance improvement is more pronounced when there is a mismatch between the LM and task domains, i.e., the non-Twitter domain tasks. 
Specifically for the \textit{PsychExp} and \textit{SCv2} datasets, sequentially unfreezing  yields significant improvement in $F_1$ building upon our intuition.

\noindent\textbf{Number of training examples.} Transfer learning is particularly useful when limited training data are available. We notice that for our largest dataset \textit{Sent17}, SiATL outperforms ULMFiT only by a small margin when trained on all the training examples available (see Table \ref{table:results}), while for the small \textit{SCv2} dataset, SiATL outperforms ULMFiT by a large margin and ranks very close to the state-of-the-art model \cite{ilic2018deep}. Moreover, the performance of SiATL vs ULMFiT as a function of the training dataset size is  shown in Figure~\ref{few}. Note that the proposed model achieves competitive results on less than 1000 training examples for the \textit{Irony18, SCv2, SCv1} and \textit{PsychExp} datasets, demonstrating the robustness of SiATL even when trained on a handful of training examples.

 \begin{figure}[!t]
 \centering
 \resizebox{\columnwidth}{!}{%
	\captionsetup{farskip=0pt} % no gap at the top
	\centerline{\includegraphics[width=1\columnwidth]{heatmap}}}
	\caption{Heatmap of the effect of $\gamma$ to $F_1$-score, evaluated on \textit{SCv2}. The horizontal axis depicts the initial value of $\gamma$ and the vertical axis the final value of $\gamma$. }
	\label{fig:heatmap}
\end{figure}




==> naaclhlt2019/tex/experimental_setup.tex <==
\vspace{-10pt}
\section{Experiments and Results} 
\subsection{Datasets}

To pretrain the language model, we collect a dataset of 20 million English Twitter messages, including approximately 2M unique tokens. We use the 70K most frequent tokens as vocabulary. We evaluate our model on five datasets: \textit{Sent17} for sentiment analysis \cite{rosenthal2017semeval}, \textit{PsychExp} for emotion recognition \cite{doi:10.1177/053901886025004001}, \textit{Irony18} for irony detection \cite{van2018semeval}, \textit{SCv1} and \textit{SCv2} for sarcasm detection \cite{DBLP:conf/sigdial/OrabyHRHRW16,lukin-walker:2013:LASM}. More details about the datasets can be found in Table \ref{table:datasets}.


% \subsection{Preprocessing} \noindent 

\subsection{Experimental Setup} \noindent

To preprocess the tweets, we use \textit{Ekphrasis}~\citep{baziotis2017datastories}. For the generic datasets, we use NLTK \cite{bird2004nltk}.
For the \textit{NBoW} baseline, we use \textit{word2vec} \cite{mikolov2013} 300-dimensional embeddings as features. For the neural models, we use an LM with an embedding size of 400, 2 hidden layers, 1000 neurons per layer, embedding dropout 0.1, hidden dropout 0.3 and batch size 32. We add  Gaussian noise of size 0.01 to the embedding layer. A clip norm of 5 is applied, as an extra safety measure against exploding gradients. For each text classification neural network, we add on top of the transferred LM an  LSTM layer of size 100 with self-attention and a softmax classification layer. For developing our models, we use PyTorch \cite{paszke2017automatic} and Scikit-learn \cite{pedregosa2011scikit}.  




==> naaclhlt2019/tex/intro.tex <==
\section{Introduction}

% \subsection{VERSION1}
Pretrained word representations captured by Language Models (LMs) have recently become popular in Natural Language Processing (NLP). Pretrained LMs encode contextual information and high-level features of language, modeling syntax and semantics, producing state-of-the-art results across a wide range of tasks, such as named entity recognition \cite{peters2017semi}, machine translation \cite{ramachandran2016unsupervised} and text classification \cite{howard2018universal}.

However, in cases where contextual embeddings from language models are used as additional features (e.g. ELMo \cite{peters2018deep}), results come at a high computational cost and require task-specific architectures. At the same time, approaches that rely on fine-tuning a LM to the task at hand (e.g. ULMFiT \cite{howard2018universal}) 
depend on pretraining the model on an extensive vocabulary and on
employing a sophisticated slanted triangular learning rate scheme  to adapt the parameters of the LM to the target dataset.

We propose a simple and effective transfer learning approach, that leverages LM contextual representations and does not require any elaborate scheduling schemes during training. 
We initially train a LM on a Twitter corpus and then transfer its weights. We add a task-specific recurrent layer and a classification layer. The transferred model is trained end-to-end using an auxiliary LM loss, which allows us to explicitly control the weighting of the pre-trained part of the model and ensure that the distilled knowledge it encodes is preserved. 

Our contributions are summarized as follows: 1) We show that transfer learning from language models can achieve competitive results, while also being intuitively simple and computationally effective. 2) We address the problem of catastrophic forgetting, by adding an auxiliary LM objective and using an unfreezing method. 3) Our results show that our approach is competitive with more sophisticated transfer learning methods.
Our code is publicly available (\href{redacted for anonymity}{will be released in future version}).	


% \subsection{VERSION2}
% Language modeling is a fundamental task in natural language processing. \st{It involves computing} \hl{LMs compute} a probability distribution over a sequence of words \st{and predicts the $(n+1)^{th}$ word, given the $n$ previous ones} \hl{, which allows to predict the most probable word to follow given the sequence}. Language models (LMs) are thus able to encode contextual information and high-level features of language, modeling syntax and semantics. These qualities make pretrained representations from LMs beneficial across a diverse set of tasks, such as named entity recognition \cite{peters2018deep, peters2017semi}, neural machine translation \cite{ramachandran2016unsupervised} and text classification \cite{howard2018universal, peters2018deep}. 

% Pretrained language representations can be used as additional features \cite{peters2018deep, mccann2017learned}, serving as contextual embeddings and being part of task-specific architectures. However, a pretrained language model can also be directly finetuned to a target task, as shown by \cite{ramachandran2016unsupervised, howard2018universal}, minimizing the modifications in the final architecture. 

% In the second case, a common problem that arises is catastrophic forgetting \cite{goodfellow2013empirical}, which results in overfitting and prevents the model from generalizing, especially when finetuned on small datasets. 

% We propose a simple and effective transfer learning approach, which leverages the contextual representations that LMs capture and, by introducing an auxiliary LM loss to the final classifier, allows controlling the pretrained part of the model and ensuring that the distilled knowledge it encodes is preserved. 

% \vspace{5pt}
% \textbf{Contributions}
% \begin{itemize}
% \item We simplify the transfer learning process proposed by \cite{howard2018universal} in text classification tasks, by integrating the LM fine-tuning step to the final model and training the classifier end-to-end.
% \item We address the problem of catastrophic forgetting, by adding an auxiliary LM objective and using an adaptive unfreezing method.
% \item We present experimental results \hl{and intuition / visualizations}, showing that our approach is competitive with more sophisticated transfer learning methods.
% \end{itemize}

% VERSION 2 ENDS HERE
% - We propose a simple one-step transfer learning method from pretrained langage models to text classification
% - We address the problem of catastrophic forgetting, by adding an auxiliary language model objective.
% - We present experimental results, showing that our approach is competitve with more sophisticated transfer learning methods.




==> naaclhlt2019/tex/model.tex <==
\section{Our Model}\label{sec:four}

We introduce \textbf{SiATL}, which stands for \textbf{Si}ngle-step \textbf{A}uxiliary loss \textbf{T}ransfer \textbf{L}earning. In our proposed approach, we first train a LM. We then transfer its weights and add a task-specific recurrent layer to the final classifier. We also employ an auxiliary LM loss to avoid catastrophic forgetting.

\vspace{4pt}

\noindent\textbf{LM Pretraining.}
We train a word-level language model, which consists of an embedding LSTM layer \cite{hochreiter1997long}, 2 hidden LSTM layers and a linear layer. We want to minimize the negative log-likelihood of the LM:
\begin{align}
L(\hat{p}) &= -\frac{1}{N}\sum_{n=1}^{N}\sum_{t=1}^{T^n} \text{log}\hat{p}(x_t^n|x_1^n,...,x_{t-1}^n)
\end{align}
where $\hat{p}(x_t^n|x_1^n,...,x_{t-1}^n)$ is the distibution of the $t^{th}$ word in the $n^{th}$ sentence given the $t - 1$ words preceding it and $N$ is total number of sentences. 
% in the corpus.
\vspace{5pt}
% We want to minimize the negative likelihood of the log probability of each training sentence:
% \begin{align}
% L_{LM} = -\mathcal{L}(\theta,D) \end{align}


\noindent\textbf{Transfer \& auxiliary loss.}
\label{transferlm}
We  transfer the weights of the pretrained model and add one LSTM with a self-attention mechanism \cite{lin2017structured,bahdanau2014neural}. 
\begin{figure}[t]
	\captionsetup{farskip=0pt} % no gap at the top
	\centering
	\includegraphics[width=1.0\columnwidth, page=1]{tiramisu}
	\caption{High-level overview of our proposed TL architecture. We transfer the pretrained LM add an extra recurrent layer and an auxiliary LM loss.}
	\label{fig:overview}
\end{figure}
\vspace{5pt}

\noindent In order to adapt the contribution of the pretrained model to the task at hand, we introduce an auxiliary LM loss during training. The joint loss is the weighted sum of the task-specific loss $L_{task}$ and the auxiliary LM loss $L_{LM}$, where $\gamma$ is a weighting parameter to enable adaptation to the target task but at the same time keep the useful knowledge from the source task. Specifically:  %The value of $\gamma$ is obtained using exponential weight decay. 
\noindent
\begin{align}
 L &= L_{task} + \gamma L_{LM}  
\end{align}
\noindent


\noindent\textbf{Exponential decay of $\gamma$.}
An advantage of the proposed TL method is that the contribution of the LM can be explicitly controlled in each training epoch.
In the first few epochs, the LM should contribute more to the joint loss of SiATL so that the task-specific layers adapt to the new linguistic distribution. After the knowledge of the pretrained LM is transferred to the new domain, the task-specific component of the loss function is more important and $\gamma$ should become smaller. In this paper, we use an exponential decay for $\gamma$ over the training epochs.
%In the first few epochs, the language model should contribute more to the joint loss of SiATL, because the new layers (LSTM and output layer) need to adapt their weights according to the probability distribution of the language model, in order to benefit from the transferred knowledge. Afterwards, the whole model should fit to the classification task. To this end, the classification loss should then weigh more. 

\vspace{4pt}

\noindent\textbf{Sequential Unfreezing.}
Instead of fine-tuning all the layers simultaneously, we propose unfreezing them sequentially, according to \citet{W18-6209}. We first fine-tune only the extra, randomly initialized LSTM and the output layer for $n-1$ epochs. At the $n^{th}$ epoch, we unfreeze the pretrained hidden layers. We let the model fine-tune, until epoch $k-1$. Finally, at epoch $k$, we also unfreeze the embedding layer and let the network train until convergence. The values of $n$ and $k$ are obtained through hyperparameter tuning. 
We find the sequential unfreezing scheme important, as it minimizes the risk of overfitting to small datasets. 



\begingroup
\setlength{\tabcolsep}{7pt} % Default value: 6pt
\renewcommand{\arraystretch}{1.1} % Default value: 1
\begin{table*}[!t]
\centering
\small
\begin{tabular}{l|c|c|c|c|c}
\Xhline{2\arrayrulewidth}
      & Irony18 & Sent17    & SCv2   & SCv1   & PsychExp \\ \hline
BoW                 & 43.7               & 61.0                & 65.1       & 60.9    &    25.8       \\
NBoW      & 45.2                & 63.0                & 61.1       & 51.9     &  20.3         
\\ \hline

P-LM  & 42.7 $\pm$ 0.6   & 61.2 $\pm$ 0.7 & 69.4 $\pm$ 0.4 &  48.5 $\pm$ 1.5 & 38.3 $\pm$ 0.3  \\

P-LM + su  & 41.8 $\pm$ 1.2 & 62.1 $\pm$ 0.8 & 69.9 $\pm$ 1.0 & 48.4 $\pm$ 1.7  & 38.7 $\pm$ 1.0 \\ \hline

P-LM + aux & 45.5 $\pm$ 0.9  & 65.1 $\pm$ 0.6 & 72.6 $\pm$ 0.7 & 55.8 $\pm$ 1.0  & 40.9 $\pm$ 0.5   \\
\textbf{SiATL} (P-LM + aux + su) & \textbf{47.0} $\pm$ 1.1 & \textbf{66.5} $\pm$ 0.2  & \textbf{75.0} $\pm$ 0.7 &\textbf{ 56.8 }$\pm$ 2.0 & \textbf{45.8} $\pm$ 1.6    \\ \hline  \hhline{======}
ULMFiT (Wiki-103)   & $23.6 \pm 1.6$      & $60.5 \pm 0.5$          &\textbf{68.7} $\pm$ 0.6   & \textbf{56.6} $\pm$ 0.5 & 21.8 $\pm$ 0.3     \\
ULMFiT (Twitter)    & \textbf{41.6} $\pm$ 0.7 & \textbf{65.6} $\pm$ 0.4   & 67.2 $\pm$ 0.9  & 44.0 $\pm$ 0.7           &  \textbf{40.2} $\pm$ 1.1    \\ \hline
\multirow{2}{*}{State of the art}  &  53.6    &  68.5  & 76.0         & 69.0       &  57.0\\ \cline{2-6} 
              &   \cite{Baziotis2018NTUASLPAS}          & \cite{cliche2017bb_twtr}   & \cite{ilic2018deep}   &  \multicolumn{2}{c}{\cite{felbo2017using}}       \\ \Xhline{2\arrayrulewidth}
\end{tabular}
\caption{Ablation study on various downstream datasets. Average over five runs with standard deviation. \textit{BoW} stands for Bag of Words, \textit{NBoW} for Neural Bag of Words. \textit{P-LM} stands for a classifier initialized with our pretrained LM, \textit{su} for sequential unfreezing and \textit{aux} for the auxiliary LM loss. In all cases, $F_1$ is employed.}
\label{table:results}
\end{table*}
\endgroup

\vspace{4pt}

\noindent\textbf{Optimizers.}
We use Stochastic Gradient Descent (SGD) for the pretrained LM with a small learning rate, in order to preserve its contextual information and avoid catastrophic forgetting. However, we want the extra LSTM and softmax layer to train fast and adapt to the target task, so in that case Adam \cite{kingma2014adam} is employed.
% We use Averaged SGD for the pretrained LM with a small learning rate ($10^{-4}$), in order to preserve its contextual information and avoid catastrophic forgetting. However, we want the extra LSTM and linear layer to adapt fast to the target task. We thus use Adam \cite{kingma2014adam} with the default learning rate for these layers.

\begin{table}[h]
\centering
\small\begin{tabular}{lccc} \Xhline{2\arrayrulewidth}
Dataset   &  Domain        & \# classes & \# examples \\ \hline
Irony18          & Tweets        & 4          & 4618        \\
Sent17          & Tweets        & 3          & 61854       \\
SCv2        & Debate Forums  & 2          & 3260        \\
SCv1               & Debate Forums & 2          & 1995        \\
PsychExp          & Experiences   & 7          & 7480   
% TREC   & Open Domain & 6 & 5500
    \\ \Xhline{2\arrayrulewidth}

\end{tabular}
\caption{Datasets used for the downstream tasks.}
\label{table:datasets}
\end{table}

==> naaclhlt2019/tex/overview.tex <==

\section{Overview}

Figure ~\ref{fig:overview} depicts a high-level overview of our approach.



==> naaclhlt2019/tex/related.tex <==
\section{Related Work}

% Transfer learning is a technique for using knowledge from a learned task to improve the performance of a related task. It was first proposed in Computer Vision \cite{torrey2010transfer, pan2010survey} to leverage knowledge learned from tasks with lots of available data in settings where few labelled data are available. 

Unsupervised pretraining has played a key role in deep neural networks, building on the premise that representations learned for one task can be useful for another task. In NLP, pretrained word vectors \cite{mikolov2013, pennington2014} are widely used, improving performance in various downstream tasks, such as part-of-speech tagging \cite{collobert2011natural} and question answering \cite{xiong2016dynamic}.

Aiming to learn from unlabeled data, \citet{dai2015semi} use unsupervised objectives such as sequence autoencoding and language modeling as pretraining representations. \citet{ramachandran2016unsupervised} also pretrain encoder-decoder pairs using language models and fine-tune them to a specific task. 
ELMo embeddings \cite{peters2018deep} are obtained from character-based bidirectional language models improving the results in a variety of tasks as additional contextual representations. 

Towards the same direction, ULMFiT \cite{howard2018universal} shows impressive results on a variety of tasks by employing pretrained LMs. The proposed pipeline requires three distinct steps, that include pretraining the LM, fine-tuning it on a target dataset with an elaborate scheduling procedure and transferring it to a classification model.


% \subsection{Auxiliary Language Model loss - Multi-Task Learning}
Multi-Task Learning (MTL) via hard parameter sharing \cite{caruna1993multitask} in neural networks has proven to be effective in many NLP problems \cite{collobert2008unified}. More recently, alternative approaches have been suggested that only share parameters across lower layers \cite{sogaard2016deep}. By introducing part-of-speech tags at the lower levels of the network, the proposed model achieves competitive results on chunking and CCG super tagging. Our auxiliary language model objective follows this line of thought and intends to boost the performance of the higher classification layer.

% Multi-Task Learning (MTL) \cite{caruana1996algorithms,caruna1993multitask, collobert2011natural} . MTL allows sharing parameters across tasks and by leveraging the correlation between related tasks, it can be beneficial for both models. Many neural network based NLP models \cite{collobert2008unified,liu2015representation}
% employ multi-task architectures, as a result of their general improvement in performance.
% In these approaches, the models share some lower layers and, after common features are determined, the rest of the layers are split into different tasks.

==> tex/overview.tex <==
\section{Overview}

Figure ~\ref{fig:overview} depicts a high-level overview of our approach.


